Provably-Correct Safety Protocol for Cooperative Platooning

Cooperative Adaptive Cruise Control (CACC) is a well-studied technology for forming string-stable vehicle platoons. Ensuring collision avoidance is particularly difficult in CACC due to the small desired inter-vehicle spacing. We propose a safety protocol preventing collisions in a provably-correct manner while still maintaining a small distance to the preceding vehicle, by utilizing communicated braking capabilities. In addition, the safety of the protocol is ensured despite possible communication failures. While our concept can be applied to any CACC system, we particularly consider a class of CACCs, where the platoon vehicles successively agree on a consensus behavior. Our safety protocol is evaluated on various scenarios using the CommonRoad benchmark suite.

==> barrier_comp.tex <==
\subsection{Barrier Computation}\label{subsec:barrier-comp}
%
The computation of the barriers for vehicle $i$ is summarized in Alg.~\ref{alg:barrier-algo}:
The barrier at a future time step is the time-wise minimum (l. 4)
over the reachable positions of the preceding vehicles (l. 3),
further restricted by the received collision positions and the sensor range (l. 2).
There, we use the input $-\infty$ to cover all behaviors of a preceding vehicle (l. 3), as no other input
can reach smaller positions according to Theorem~\ref{prop:monotonicity}.
%
%
\algrenewcommand\algorithmicindent{0.9em}%
\begin{algorithm}
\small
\caption{Barrier computation for vehicle $i$}
\label{alg:barrier-algo}
\textbf{Input:} Preceding vehicles $\X=\{i+1 \dots N\}$,
set $\SRestr_{\text{coll}}$ of received collision positions \\
\textbf{Output:} Barriers $\lb{s}_k$ for $i$
\begin{algorithmic}[1]
\Procedure{CompBarriers}{$\X$}
\State $\SRestr \gets \SRestr_{\text{coll}} \cup \{\sensorrange\} $ \Comment{barriers at any time}
\vtab \For{$j \in \X$}: $\of{\lb{s}}{j}_{k} \gets \lowerpos{j}(-\infty)$ \Comment{cf. \eqref{eq:lowerpos} }
\EndFor
\State $\lb{s}_k \gets
( \min(
    \Set{
        \of{\lb{s}}{j}_{k}
    }{
        j\in \X
    } \cup \SRestr)
    )_{k=0}^{\infty}$
\State \Return $\lb{s}_k$
\EndProcedure
\end{algorithmic}
\end{algorithm}
%

==> fail_safe.tex <==
\subsection{Fail-Safe Controller}\label{subsec:fail-safe}
While our fail-safe maneuver is principally a full brake (cf. l. 3 in Alg.~\ref{alg:safety-algo}),
we additionally incorporate a fail-safe controller (cf. l. 6 in Alg.~\ref{alg:overall-algo}) in case the nominal
input is unsafe to avoid full braking whenever possible.
This is realized by computing the maximum acceleration that is still safe.

To this end, our fail-safe controller computes the barriers $\lb{s}_k \gets \Call{CompBarriers}{\X}$ for $i$.
It then approximates the root of the following function $f$ with precision $a_{\text{tol}}$ using
binary search, resulting in $a^*$:
\begin{equation}
\begin{aligned}
f(a) = \min_{k \in \{0 \dots \infty\} } \lb{s}_k - (\upperpos{i}(a(\cdot)))_{k+1} \text{,}
\end{aligned}
\end{equation}
%
\begin{equation*}
\begin{aligned}
\text{where}~a(\cdot)~\text{is defined by}~a(t') \gets \begin{cases}
          a & \text{if}~t' \leq \tplanning  \\
          -\infty & \text{otherwise}\text{.}
      \end{cases} \\
\end{aligned}
\end{equation*}
%
If $f$ has a root $a^*$, the resulting acceleration is $\of{a_d}{i} = a^* - a_{\text{tol}}$,
which is guaranteed to be a safe input and is the least harsh one doing so up to $a_{\text{tol}}$.
If $f$ does not have a root, no safe input exists, and $\of{a_d}{i}=-\infty$ is returned to mitigate
the imminent collision.
%The return value $\text{safe}$ indicates whether a safe acceleration was found.
A particular advantage of this controller is that it can be executed anytime-like in parallel to the nominal CACC,
by successively decreasing $a_{\text{tol}}$.
% as long as computation time is left for the current planning step, which results in a less conservative
% acceleration over time that is still always safe.
%

==> recap.tex <==
\subsection{Recapturing Controller}\label{subsec:recap}
% Hint: Difference to Safe ACC: we do not need any precomputation for being real-time capable. This is done by
% considering the whole time until standstill in the QP and not only the time until safe distance is recaptured.
% Precomputing things would be bad for us, as the ego acceleration limit changes over time in the consensus case.
% Furthermore, the precomputation makes the result less accurate due to discretization of the safe distance at the end.
The recapturing controller (line 5 in Alg.~\ref{alg:overall-algo}) provides a smooth reaction of vehicle $i$ to a
cut-in of vehicle $j$, by minimizing the jerk during the remaining clearing time.
We define the number of planning steps during the remaining clearing time by $z=\floor{\frac{\tclearrem{j}}{\tplanning}}$.
Using MPC, a discrete jerk profile $(\jerk)_{k=1}^{n}$ is computed,
where $n$ is chosen in a way such that $i$ is able to stop within $n\tplanning$.
$\jerk_k$ is transformed to a piece-wise constant acceleration trajectory
$(a)_{k=0}^{n}$ by
%
\begin{equation*}
\begin{aligned}
& a_{k} = \begin{cases}
        \of{a}{i}(t-\tplanning)~\text{if}~k=0 \\
        a_{k-1}+\tplanning\jerk_{k}~\text{otherwise}\text{.}
    \end{cases}
\end{aligned}
\end{equation*}
%
We define the sequences $(s)_{k=0}^n$ and $(v)_{k=0}^n$ by simulating $a_{k}$ forward in time, starting from
$\vectorhoriz{s_0 & v_0}\coloneqq\xofupper{i}{t}$ and using a simple point mass model.
%
We write $\jerk_{1:z}$ for the vector with the first $z$ elements of $\jerk_k$.
With that, $\jerk_{k}$ is computed by solving the following quadratic program using the batch approach described
in~\cite[Chapter~8.2]{borrelli_predictive_nodate}:
%
\begin{equation}\label{eq:recap}
\begin{aligned}
% Hint: why will different costs for the different times (i.e. higher cost for nearer time steps) not be useful?
%   --> as we minimize the jerk, this will result in stronger accelerations only later in the future anyways
\min_{\jerk_{k}} \jerk_{1:z}^T\jerk_{1:z}
\end{aligned}
\end{equation}
%
s.t. $\forall k \in \{0 \dots n-1\}$:
%
\begin{equation}\label{eq:behind}
\begin{aligned}
\front{i}(s_{k+1}) \leq \of{\lb{s}}{j}_{k} \text{,}
\end{aligned}
\end{equation}
%
\begin{equation}\label{eq:v-constraint}
\begin{aligned}
% Hint: the constraint 0 <= v_{k+1} is not necessary here; if velocity goes below 0 during solving the simulated
%   input trajectory, that's fine: then the input trajectory leads the ego to standstill, and if the position
%   constraints were fulfilled until then, we are done.
v_{k+1} \leq \vmax{i} \text{,}
\end{aligned}
\end{equation}
%
\begin{equation}\label{eq:a-constraints}
\begin{aligned}
\aminforce{i} \leq a_{k+1} \leq \amaxforce{i}~\text{and}
\end{aligned}
\end{equation}
%
\begin{equation}\label{eq:finallystop}
\begin{aligned}
v_n \leq 0 \text{.}
\end{aligned}
\end{equation}
%
Here, $\of{\lb{s}}{j}_{k}=\lowerpos{j}(t, -\infty,\aminforce{j})$, i.e., Constraint~\eqref{eq:behind}
ensures that $a_k$ keeps $i$ behind $j$.
Constraints~\eqref{eq:v-constraint} and~\eqref{eq:a-constraints} are for considering the state and input bounds,
and constraint~\eqref{eq:finallystop} ensures that $a_k$ makes $i$ finally stop.
The recapturing controller then returns $a_{1}$.

By limiting $\of{a_d}{i}$ above $a_{1}$ (line 8 in Alg.~\ref{alg:overall-algo}),
we try to prevent that $i$ has to make abrupt changes in its acceleration later to recapture the safe distance
within $\tclearrem{j}$.
In contrast to~\cite{althoff_provably-correct_2021}, we consider the whole time until $i$ stops rather than
only the remaining clearing time.
By that, pre-computing solutions offline is not necessary, which is favorable when using a consensus
protocol leading to changes in the braking limits and, thus, to changes in the solutions.
% Hint: By minimizing the safe distance, we accept that the ego vehicle fully brakes if the preceding vehicle does so.
%   But: in the case of a cut-in, the relaxed assumed behavior of vehicle j is more realistic (i.e. the input of j
%   will be close to our assumptions more likely) --> thus, if we just normally verify a_t, then it is likely that i
%   has to fully brake in the next time step --> more precisely: i has to fully brake if j behaves as we assumed.
%   But: this is in general bad. Better would be, if the ego vehicle brakes stronger immediately to prevent a full
%   brake later on.
%
% Note that $\jerk_{\text{recap},k}$ is only minimized during the remaining clearing time, i.e. for $z$ time steps,
% which is technically realized using a small cost factor for $k > z$.
% Further, note that the acceleration constraint in~\eqref{eq:recap-a-constraints} does not consider the road incline
% and air drag; thus, $a_{\text{recap},1}$ is not guaranteed to be a safe input for the current time step.
% However, this does not impede safety, as the resulting overall acceleration is verified in lines $14-17$ in
% Alg.~\ref{alg:overall-algo} again.
% This is how the forward simulation is done exactly:
% \begin{equation*}
% \begin{aligned}
% \vectorhoriz{s_k & v_k & a_k} = \begin{pmatrix}
%                                 1 & \tplanning & 0.5\tplanning \\
%                                 0 & 1 & \tplanning \\
%                                 0 & 0 & 1
%                                 \end{pmatrix} \cdot \vectorhoriz{s_{k-1} & v_{k-1} & a_{k-1} }
%                                 + \jerk \vectorhoriz{ 0.5\tplanning^3 & \tplanning^2 & \tplanning }
% \end{aligned}
% \end{equation*}
%   --> we actually apply the jerk to the acceleration for \Delta t and then apply the new acceleration to the state!!
%   --> that's why this is different to when j is constant for \Delta t but a is not

==> recap_and_failsafe.tex <==
\section{RECAPTURING AND FAIL-SAFE CONTROLLER}\label{sec:recap_and_fail_safe}
%
\input{recap_short.tex}
%
\input{fail_safe.tex}

==> recap_short.tex <==
\subsection{Recapturing Controller}\label{subsec:recap}
The recapturing controller (line 3 in Alg.~\ref{alg:overall-algo}) provides a smooth reaction of vehicle $i$ to a
cut-in of vehicle $j$.
It is similar to the one proposed in~\cite[Sec. V.B.2)]{althoff_provably-correct_2021}.
Using Model Predictive Control, it computes a piece-wise constant input trajectory that
a) minimizes jerk during the remaining clearing time,
b) brings $i$ eventually to a standstill, and c) keeps $i$ behind the sequence $\lowerpos{j}(-\infty,\aminforce{j})$.
The result $a_{\text{recap}}$ of the recapturing controller is the first acceleration of that trajectory.
By limiting $\of{a_d}{i}$ above $a_{\text{recap}}$ (line 4 in Alg.~\ref{alg:overall-algo}),
we try to prevent that $i$ has to make abrupt changes in its acceleration later to recapture the safe distance
within the remaining clearing time.
In contrast to~\cite{althoff_provably-correct_2021}, we consider the whole time until $i$ stops rather than
only the remaining clearing time.
By that, pre-computing solutions offline is not necessary, which is favorable when using a consensus
protocol leading to changes in the braking limits and, thus, to changes in the solutions.
%% Original pseudo-code, invoking the recap controller for all cut-in vehicles:
%\State $a_{\min,\text{recap}} \gets \infty$

%\For{$j \in \Set{k \in X}{\tclearrem{k} > 0}$}: \Comment{$j$ is cut-in vehicle}
% if i is always below j, they are possibly safe at the moment
%    \State $a_{\text{recap}} \gets \Call{Recap}{i, j}$ \Comment{Sec.~\ref{subsec:recap}}
%    \State $a_{\min,\text{recap}} \gets \min(a_{\min,\text{recap}}, a_{\text{recap}})$
%\EndFor

==> scoll.tex <==
\subsection{Collision Position Prediction}\label{subsec:scoll}
%
In case of an imminent collision, we predict the position of the ego vehicle $i$ at the time of collision by
determining the first time step $k_{\text{coll}}$, at which $i$ hits its barriers $\lb{s}_{k} = \Call{CompBarriers}{\X}$.
As $i$ performs a full brake if a collision impends (cf. Sec.~\ref{subsec:fail-safe}), its reachable positions are
bounded by the sequence $\of{\overline{s}}{i}_{k} = \upperpos{i}(-\infty)$.
Thus, $k_{\text{coll} } = \min( \Set{k \geq 0}{ \of{\overline{s}}{i}_{k+1} \geq \lb{s}_{k}  } )$, and the corresponding
rear position of $i$ is $\scoll = \of{\overline{s}}{i}_{k_{\text{coll}}} - \of{l}{i}$.

==> verification_procedure.tex <==
\subsection{Verification Procedure}\label{subsec:verification-procedure}
%
The overall procedure of verifying safety for a planned input is shown in Alg.~\ref{alg:safety-algo}.
Here, we use the input $-\infty$ for the fail-safe maneuver of vehicle $i$ after $a_d$
(l. 3), as no other input can reach smaller positions according to Theorem~\ref{prop:monotonicity}.
Note that we compare the $k+1$-th upper bound of the reachable ego position with the $k$-th barrier (l. 5),
such that we
can exclude a collision within each future time interval $[k\tplanning,(k+1)\tplanning]$.
%
%

